Arbitrary order stationarity preserving stabilized finite elements for multidimensional nonlinear hyperbolic problems. Application to the Euler equations with gravity

We develop arbitrarily high-order, stationarity-preserving stabilized finite element methods for multidimensional nonlinear hyperbolic balance laws on Cartesian grids. We aim at approximating all the steady states of the problem at hand, including non-trivial genuinely multidimensional equilibria, with a level of accuracy higher than the nominal one of the underlying scheme. We formalize more precisely the meaning of stationarity preservation, providing some technical conditions for its realizability. We then recast the multidimensional global-flux quadrature of Barsukow et al. (Num. Meth. PDEs, 2025) as a local preprocessing of the physical fluxes that maps continuous polynomial vector fields to a local space with Raviart--Thomas-type structure. Both the Galerkin and SUPG formulations are recast in this setting. The resulting methods extend the stationarity-preserving finite-volume approach of Barsukow et al. (J. Comput. Phys., 2026) to high-order continuous finite elements and Barsukow et al. (Num. Meth. PDEs, 2025) to nonlinear balance laws. We analyze key properties of the proposed schemes, including local conservation and nodal superconvergence of the discrete steady kernel, and we discuss their relation to low-Mach-compliant discretizations. We apply the framework to the compressible Euler equations with gravity. A simple source-term reformulation yields machine-precision preservation of isothermal hydrostatic equilibria. Extensive numerical benchmarks, including moving equilibrium, near-equilibrium, and instability-dominated regimes, demonstrate clear improvements in robustness and accuracy over standard SUPG and reference finite-volume methods.

==> section21.tex <==
\section{Systems of balance laws}

\begin{itemize}
\item  notation for a generic system 
\item exaxmples used in the paper 
\end{itemize}

\subsection{Multi-Dimensional Nonlinear Hyperbolic Balance Laws}
We focus on the numerical resolution using a new method called Streamline Upwind Petrov–Galerkin with Global Flux Quadrature (SUPG-GFQ), applied to hyperbolic systems of conservation laws with source terms, which can be written in the following form:
\begin{equation}
	\frac{\partial \bm{W}}{\partial t} + \frac{\partial \bm{F}(\bm{W})}{\partial x} + \frac{\partial \bm{G}(\bm{W})}{\partial y} = \mathbf{S}(\bm{W}),
\end{equation}
can be written in a quasi-linear form:
\begin{equation}
	\partial_t \bm{W} + \mathbf{J}_F \, \partial_x \bm{W} + \mathbf{J}_G \, \partial_y \bm{W} = \mathbf{S}(\bm{W}),
\end{equation}
where $\mathbf{J}_F$ and $\mathbf{J}_G$ are the Jacobian matrices of the fluxes $\bm{F}$ and $\bm{G}$, respectively. They are defined as:
\begin{equation}
	\mathbf{J}_F := \frac{\partial \mathbf{F}(\bm{W})}{\partial \bm{W}}, \qand
	\mathbf{J}_G := \frac{\partial \mathbf{G}(\bm{W})}{\partial \bm{W}}.
\end{equation}

 
\subsubsection{Compressible Euler Equations with gravitational effects}

The compressible Euler equations describe the motion of an ideal gas in the absence of viscosity and thermal conduction. They can be seen as a simplification of the Navier–Stokes equations and are widely used in the simulation of high-speed compressible flows, such as those encountered in aerodynamics or astrophysics.

The equations express the conservation of mass, momentum, and total energy. In vectorial form, the system reads:
\begin{equation}\label{Euler_Eq}
\begin{cases}
	\partial_t \rho + \nabla \cdot (\rho \mathbf{u}) = 0, \\
	\partial_t (\rho \mathbf{v}) + \nabla \cdot (\rho \mathbf{u} \otimes \mathbf{u}) + \grad{p} = -\rho \grad {\phi}, \\
	\partial_t (\rho E) + \nabla \cdot (\rho H \mathbf{u}) = -\rho \mathbf{u} \cdot \grad{\phi},
\end{cases}
\end{equation}
where $\rho$ denotes the fluid density, $\mathbf{u}$ the velocity vector, $E$ the specific total energy given by \(E = \rho(e + \frac{1}{2}|\mathbf{u}|^2)\), $H = E + \frac{p}{\rho}$ the total specific enthalpy and $\Phi$ the gravitational potential. The pressure is related to the internal energy through the equation of state for a perfect gas: \(p = (\gamma - 1)\rho e\), with $\gamma$ the ratio of specific heats (e.g., $\gamma = 1.4$ for air).

This system can also be recast in conservative form with:
\begin{equation}
	\bm{W} =
	\begin{pmatrix}
		\rho \\
		\rho u \\
		\rho v \\
		\rho E
	\end{pmatrix}, \qquad
	\mathbf{F} (\bm{W}) =
	\begin{pmatrix}
		\rho u \\
		\rho u^2 + p \\
		\rho u v \\
		\rho u H
	\end{pmatrix}, \qquad
	\mathbf{G} (\bm{W}) =
	\begin{pmatrix}
		\rho v \\
		\rho u v \\
		\rho v^2 + p \\
		\rho v H
	\end{pmatrix},
\end{equation}
and source terms s are given by
\begin{equation}
	\mathbf{S}(\bm{W}) =
	\begin{pmatrix}
		0 \\[0.5em]
		- \rho \, \dfrac{\partial \phi}{\partial x} \\[0.5em]
		- \rho \, \dfrac{\partial \phi}{\partial y} \\[0.5em]
		- \rho \left( u \, \dfrac{\partial \phi}{\partial x} + v \, \dfrac{\partial \phi}{\partial y} \right)
	\end{pmatrix}.
\end{equation}
The Jacobian matrices associated with the fluxes \(\mathbf{F}\) and \(\mathbf{G}\) are given by:
\begin{equation}
	\mathbf{J}_F =
	\begin{pmatrix}
		0 & 1 & 0 & 0 \\
		(\gamma - 1)\dfrac{q^2}{2} - u^2 & (3 - \gamma)u & (1 - \gamma)v & \gamma - 1 \\
		-uv & v & u & 0 \\
		\left(\gamma - 1\right)\left( \dfrac{q^2}{2} - H \right)u & H + (1 - \gamma)u^2 & (1 - \gamma)uv & \gamma u
	\end{pmatrix},
\end{equation}

\begin{equation}
	\mathbf{J}_G  =
	\begin{pmatrix}
		0 & 0 & 1 & 0 \\
		-uv & v & u & 0 \\
		(\gamma - 1)\dfrac{q^2}{2} - v^2 & (1 - \gamma)u & (3 - \gamma)v & \gamma - 1 \\
		\left(\gamma - 1\right)\left( \dfrac{q^2}{2} - H \right)v & (1 - \gamma)uv & H + (1 - \gamma)v^2 & \gamma v
	\end{pmatrix},
\end{equation}
where $q^2 = u^2 + v^2$.  
Although the Euler equations admit more complex equilibrium configurations than simpler systems such as the shallow water equations, they can still be characterized by specific balance conditions. In particular, steady states satisfy
\begin{equation}
	\nabla \cdot (\rho \mathbf{u}) = 0, \qquad
	(\rho \mathbf{u} \cdot \nabla)\mathbf{u} + \nabla p = 0, \qquad
	\mathbf{u} \cdot \nabla H = 0,
\end{equation}
which correspond respectively to mass conservation, momentum balance, and constancy of the total enthalpy along streamlines. 

When gravitational effects are included, the Euler equations also admit hydrostatic equilibrium solutions, provided the following conditions hold:
\begin{equation}
	\mathbf{u} \equiv 0, 
	\qquad \nabla p = - \rho \nabla \phi,
\end{equation}
As system~(\ref{Euler_Eq}) does not contain any dissipative terms, steady states may only occur if they are compatible with the initial and boundary conditions. In addition, the following compatibility condition

\begin{equation}
	\nabla \times (\rho \nabla \phi) = 0
\end{equation}
must be satisfied to ensure the existence of a hydrostatic equilibrium. 

Identifying and preserving such equilibria is crucial in many physical applications, particularly in flows close to equilibrium where spurious numerical errors can dominate the true dynamics.



